Sequential Drift Detection in Deep Learning Classifiers

We utilize neural network embeddings to detect data drift by formulating the drift detection within an appropriate sequential decision framework. This enables control of the false alarm rate although the statistical tests are repeatedly applied. Since change detection algorithms naturally face a tradeoff between avoiding false alarms and quick correct detection, we introduce a loss function which evaluates an algorithm's ability to balance these two concerns, and we use it in a series of experiments.

==> related.tex <==
\section{Related work} \label{sec:related}

% In practice one may attempt to determine if the distribution of the data has changed accepting the fact that false alarms may result from identifying distribution changes that are not impacting the network performance.  Empirical density estimation has been well investigated and a variety of approaches exist for the classical settings in which the data has low dimensionality or is drawn from a known  distribution or mixture of distributions. 

% It has also been acknowledged that density estimation becomes very challenging for high-dimensional data \cite{Scholkopf:2001:ESH:1119748.1119749}. 
% Modeling multivariate data with Bayesian networks is one example for a domain that has been struggling with this challenge \cite{SMITH2003387}. 

% Earlier work have proposed high dimensionality density estimation, such as Maximum Mean Discrepancy \cite{Gretton:2012:KTT:2188385.2188410} or Wasserstein distance \cite{OLKIN1982257}. 
% However, statistical calculations like a confidence interval, which depend on the distribution, become much more complicated for high dimension metrics than uni-variate metrics. Further, as the dimensionality increases so does the likelihood of having insufficient data for reliably performing such statistical calculations.

% In \cite{orna19} drift detection is attempted using a uni-variate machine learning model confidence interval as a statistics.  This work is black box -- it applies to any machine learning approach that produces a confidence number but does not take advantage of the inner structure of the machine learning model.  In contrast, given the importance of neural networks, we drive new statistics that take advantage of the structure of the network but follow \cite{orna19} and collapsing the statistic we apply to a uni-variate statistic avoiding thus avoiding the curse of high dimensions incurred when attempting to approximate the distribution directly.   

% Another approach to the change in data distribution is to increase the robustness of the model so that it better handle changes in the data, identify data missing from the training examples or identify bias in the training examples. Such approaches often focus on handling missing data or direct learning to areas in the data where the model performs poorly.  Ensembles of weak learners such as AdaBoost are an example. Further research is needed to analyze the relation between such approaches, distribution drift and model performance drift.   

% Various work captures challenges and best practices in developing ML solutions, e.g., \cite{Google_technical_debt,Google_testscore,Google_43rules}.
% Interestingly model performance drift is not addressed by this work.   Our research deals with capturing the expected envelope of operation of a network and monitoring for significant changes against it. The approach is especially important when the production data is not labeled which is the case in many business applications.

In this work, the sequential test was applied on the similarity measure of outputs from our neural network model, since the raw data are difficult to analyze directly.  Assuming that the output metric reflects changes in the underlying data, this technique should be successful in generalizing such potentially complex drift detection problems to a univariate problem. We have done previous work on detecting inserted drift (e.g. other digits images, out-of-class images) in images observed over time from the MNIST dataset by monitoring changes in our machine learning model that was trained on the un-contaminated data.  This work was presented in the 2019 annual Israel Statistical Association conference, and will be presented in the 2020 Joint Statistical Meetings (JSM). 
